Federated Learning for Healthcare Domain - Pipeline, Applications and Challenges

Federated learning is the process of developing machine learning models over datasets distributed across data centers such as hospitals, clinical research labs, and mobile devices while preventing data leakage. This survey examines previous research and studies on federated learning in the healthcare sector across a range of use cases and applications. Our survey shows what challenges, methods, and applications a practitioner should be aware of in the topic of federated learning. This paper aims to lay out existing research and list the possibilities of federated learning for healthcare industries.

==> text.tex <==
\begin{document}

\usepackage{tabularx}

\begin{table*}[!t]
\caption {Test
}\label{Tab:dcnnarchitectures}
\centering
\renewcommand{\arraystretch}{1.2}
\setlength\arrayrulewidth{0.2mm}
\setlength\tabcolsep{2pt}
\resizebox*{16cm}{!}{
\begin{tabular}{p{6 cm}cccp{6cm}}
\Xhline{1pt}

\footnotesize Title & \footnotesize Ref & \footnotesize Year & \footnotesize Category &\footnotesize Content \\
\Xhline{1pt}

\hline

{\footnotesize Variation-Aware Federated Learning with Multi-Source Decentralized Medical Image Data } 
& \raisebox{-3.3ex}[0pt]{\footnotesize \cite{Girshick2014RCNN}} 
& \raisebox{-3.3ex}[0pt]{\footnotesize 2021} & \raisebox{-3.3ex}[0pt]{\footnotesize \shortstack [c] {Learning \\ Systems}} 
& \footnotesize Variation-aware federated learning (VAFL) is a methodology proposed in this research for minimising client variations by transforming all clients' images into a shared image space \\



\hline

{\footnotesize Federated Learning in a Medical Context: A Systematic Literature Review } 
& \raisebox{-3.3ex}[0pt]{\footnotesize \cite{Girshick2014RCNN}} 
& \raisebox{-3.3ex}[0pt]{\footnotesize 2021} & \raisebox{-3.3ex}[0pt]{\footnotesize Survey} 
& \footnotesize This survey article examines federated learning and its relevance to sensitive healthcare data \\

\hline

{\footnotesize Federated Learning for Smart Healthcare: A Survey } 
& \raisebox{-3.3ex}[0pt]{\footnotesize \cite{Girshick2014RCNN}} 
& \raisebox{-3.3ex}[0pt]{\footnotesize 2021} & \raisebox{-3.3ex}[0pt]{\footnotesize Survey} 
& \footnotesize The application of FL in smart healthcare and IoT devices are reviewed and surveyed in this survey report \\




\Xhline{1pt}
\end{tabular}
}
\end{table*}

\end{document}
